Modeling Latent Sentence Structure in Neural Machine Translation

Recently it was shown that linguistic structure predicted by a supervised parser can be beneficial for neural machine translation (NMT). In this work we investigate a more challenging setup: we incorporate sentence structure as a latent variable in a standard NMT encoder-decoder and induce it in such a way as to benefit the translation task. We consider German-English and Japanese-English translation benchmarks and observe that when using RNN encoders the model makes no or very limited use of the structure induction apparatus. In contrast, CNN and word-embedding-based encoders rely on latent graphs and force them to encode useful, potentially long-distance, dependencies.

==> fig_graphical_model.tex <==
% FIGURE: Graphical Model
\begin{figure}[tb]
\centering
\begin{tikzpicture}
% Define nodes
\node[obs,fill=gray!75]    (x) {$ x_1^m $};
\node[latent, right=of x]   (h) {$ h $};
\node[obs, above=of h]     (y) {$ y $};
\node[obs, left=of y]  (pre-y) {$ y_< $};
\node[latent,right=of h] (pre-h) {$ h_< $};

% Connect nodes
\edge{x}{h,y};
\edge{h}{y};

\edge{pre-y}{y};
\edge{pre-h}{h};

\plate{y-sentence}{(pre-y)(y)}{$n$};
\plate{h-sentence}{(pre-h)(h)}{$m$};

% add plates
\end{tikzpicture}
\caption{\label{fig:pgm}Conditional independences.}
\end{figure}

